Ditch the Gold Standard: Re-evaluating Conversational Question Answering

Conversational question answering aims to provide natural-language answers to users in information-seeking conversations. Existing conversational QA benchmarks compare models with pre-collected human-human conversations, using ground-truth answers provided in conversational history. It remains unclear whether we can rely on this static evaluation for model development and whether current systems can well generalize to real-world human-machine conversations. In this work, we conduct the first large-scale human evaluation of state-of-the-art conversational QA systems, where human evaluators converse with models and judge the correctness of their answers. We find that the distribution of human machine conversations differs drastically from that of human-human conversations, and there is a disagreement between human and gold-history evaluation in terms of model ranking. We further investigate how to improve automatic evaluations, and propose a question rewriting mechanism based on predicted history, which better correlates with human judgments. Finally, we analyze the impact of various modeling strategies and discuss future directions towards building better conversational question answering systems.

==> sections/Discussion.tex <==
%!TEX root = ../main.tex

\section{Discussion}\label{sec:discussion}
\subsection{Unanswerable Questions}
\subsection{History modeling}
\paragraph{Effect of Question Rewriting}

\paragraph{Effect of using answer text versus answer span marker in conversation history}


==> sections/Models.tex <==
%!TEX root = ../main.tex

\section{Modeling Question and History}\label{sec:models}

\begin{figure}[ht!]
    \centering
    \begin{subfigure}{.45\columnwidth}
        \centering
        \includegraphics[width=.8\textwidth]{figures/BERT.png}
        \caption{BERT}
        \label{subfig:bert}
    \end{subfigure}
    \begin{subfigure}{.45\columnwidth}
        \centering
        \includegraphics[width=.8\textwidth]{figures/HAM.png}
        \caption{HAM}
        \label{subfig:ham}
    \end{subfigure}
    \newline
    \begin{subfigure}{.45\columnwidth}
        \centering
        \includegraphics[width=.8\textwidth]{figures/ExCorD.png}
        \caption{ExCorD}
        \label{subfig:excord}
    \end{subfigure}
    \begin{subfigure}{.45\columnwidth}
        \centering
        \includegraphics[width=.8\textwidth]{figures/GraphFlow.png}
        \caption{GraphFlow}
        \label{subfig:gf}
    \end{subfigure}
    \caption{Model Structures}
    \label{fig:model_structures}
\end{figure}

% \tianyu{I'm not sure where those should be put. The intro of the models are very detailed and long, so if we have this long section before the analysis result readers may get tired even before reaching the important content.}

The four models we used for experiments in Section~\ref{sec:analysis} have varied performance regarding answerable and unanswerable questions. In this section, we attempt to give explanations for the models' behaviors, with the hope of shedding light on the most appropriate model structures for the CQA task.

\subsection{Baseline Models}\label{subsec:models_baselines}
We use the following models as our baselines for comparison:

\paragraph{\bert.} We borrowed the architecture from ~\citet{ohsugi2019simple} and implemented our own model by modifying the code from Bert4CoQA repository \footnote{https://github.com/adamluo1995/Bert4CoQA}. The best model is trained with \ttt{BERT-base-uncased}.

\paragraph{\ham.} \citet{qu2019attentive} added a history attention mechanism (HAM) to conduct a "soft selection" for conversation histories. They also use multi-task learning (MTL) to do dialog act prediction and answer type prediction in addition to answer prediction. We use their best reported model from CodaLab trained with \ttt{BERT-large-uncased}.

%This method attends to history turns with different weights based on how helpful they are on answering the current question. In addition to handling conversation history, they also use multi-task learning (MTL) to do answer prediction along with another essential conversation task (dialog act prediction and answer type prediction) using a uniform model architecture. We use their best reported model from CodaLab trained with \ttt{BERT-large-uncased}.

\paragraph{\excord.} \citet{kim2021learn} used pairs of original and rewritten self-contained questions to train the QA model with a consistency-based regularizer. The self-contained questions come from a T5-based sequence generator~\cite{raffel2020exploring} finetuned on the CANARD dataset. We use their best reported model, which was trained with \ttt{RoBERTa-base}.
% Instead of an end-to-end approach, \citet{kim2021learn} separately train a question rewriting model and a question answering model. They first use a T5-based sequence generator~\cite{raffel2020exploring} as their QR model, which generates self-contained questions that can be understood without the conversation history. They then used the pairs of original and rewritten self-contained questions to train the QA model with a consistency-based regularizer. We use their best reported model, which was trained with \ttt{RoBERTa-base}.

\paragraph{graphflow}
\citet{chen2019graphflow} use a Recurrent GNN model with BERT embeddings. They use a graph structure learning technique to dynamically construct a question and conversation history aware context graph at each conversation turn. They also include a flow mechanism to model the temporal dependencies in a sequence of context graphs. We followed their approach and hyperparameters to reproduce their best result, also using their data that had been preprocessed into graph structure.

\subsection{Question Encoding} \label{subsec:models_question}

\paragraph{BERT.} For each turn, we augment the current question with the question-answer pairs of the previous two turns, and then prepend the augmented question to the context. We then feed the sequence into BERT and BERT generates contextualized token-level representations for each sequence with token type embedding, segment embedding and positional embedding. We use a sliding window approach to split long passages, and thus construct multiple input sequences for a given question.

\paragraph{HAM.} For each turn, they prepend the original question to the context and then feed the sequence into BERT, where BERT generates contextualized token-level representations for each sequence based on the embeddings for tokens, segments, positions, and a special positional history answer embedding (PosHAE). The procedure of generating PosHAE is detailed in Section~\ref{subsec:models_history}.

\paragraph{ExCorD.} During training, they pair self-contained questions with the original question to perform consistency regularization, enforcing the model’s predicted answers from the original questions to be similar to those from the self-contained questions. For the majority of self-contained questions, they use the rewritten questions from the CANARD dataset, and use a \ttt{T5} Question-Rewriting model trained on CANARD dataset to rewrite the rest of training questions. Their consistency loss is defined as:
\begin{equation}
\resizebox{.85\hsize}{!}{%
$
    \mathcal{L}_t^\text{cons} = \text{KL}(\mathrm{P}^\text{read}_{\theta}(a_t|d,q_t,\mathcal{H}_t)||\mathrm{P}^{\text{read}}_{\bar{\theta}}(a_t|d,\tilde{q}_t,\tilde{\mathcal{H}}_t))
\label{equation:consistency_reg}
$}
\end{equation}
where $\text{KL}(\cdot)$ represents the Kullback–Leibler divergence function between two probability distributions. $\theta$ is the model's parameters, and $\bar{\theta}$ depicts a fixed copy of $\theta$. $q_t$ means the original question while $\tilde{q}_t$ denotes the self-contained question. $\mathcal{H}_t$ means the conversational history constructed with original questions and $\tilde{\mathcal{H}}_t$ denotes the conversational history constructed with self-contained questions. $\mathrm{P}^\text{read}_{\theta}(a_t|\cdot)$ is the answer span distribution over all evidence document tokens. Their final training loss is calculated as:

\begin{equation}
 \mathcal{L} =  \mathcal{L}^\text{orig} + \lambda_1 \mathcal{L}^\text{self} + \lambda_2 \mathcal{L}^\text{cons}
\label{equation:total_loss}
\end{equation}
\noindent where $\lambda_1$ and $\lambda_2$ are hyperparameters.
$\mathcal{L}^{\text{orig}}$ and $\mathcal{L}^{\text{self}}$ are calculated by the negative log-likelihood between the predicted answers and gold standards given the original and self-contained questions, respectively.

During testing, only original questions are used.

\paragraph{GraphFlow.} For each turn, for each context word $c_j$, they incorporate an aligned question embedding
\begin{equation*}
\begin{aligned}
f_{align}(c_{j})=\sum_{k}{\beta_{j,k} \mf{g}_{k}^{Q}}
\end{aligned}
\end{equation*}
where $\mf{g}_{k}^{Q}$ is the GloVe embedding of the $k$-th question word $q_k$ and $\beta_{j,k}$ is an attention score between context word $c_j$ and question word $q_k$.
The attention score $\beta_{j,k}$ is computed by
\begin{equation*}
\begin{aligned}
\beta_{j,k} \ \propto \ \text{exp}(\text{ReLU}(\mf{W} \mf{g}_{j}^C)^T \text{ReLU}(\mf{W} \mf{g}_{k}^{Q}))
\end{aligned}
\end{equation*}
where $\mf{W}$ is a $d \times 300$ trainable weight with
$d$ being the hidden state size, and $\mf{g}_{j}^C$ is the GloVe embedding of context word $c_j$.



\subsection{Conversation History Modeling} \label{subsec:models_history}

\paragraph{BERT.} Following ~\citet{ohsugi2019simple}, we prepend two question-answer pairs to the current question, which is then prepended to the context, and feed the resulting sequence into the BERT encoder. For questions that do not have two previous turns, we prepend the most number of previous turns in the conversation history.

\paragraph{HAM.} HAM employs two methods for modeling conversation history.The first method is \tf{Positional History Answer Embedding (PosHAE)}, which is an embedding that will be fed into the BERT encoder along with token type, segment and positional embeddings. The PosHAE is created following the procedure below:

\begin{enumerate}
    \item Given the current question $q_k$ and a history turn $H_k^i$, compute the relative position of $H_k^i$ in terms of $q_k$ as $k-i$.
    \item For each token in the current contextualized question $q_k$, its vocabulary ID is $k-i$ if the token appeared in history turn $H_k^i$, and 0 if it did not.
    \item Use a truncated normal distribution to initialize an embedding look up table \tf{ET} $\in \mb{R}^{|I+1| \times h}$, then use the vocabulary ID to map each token to a history answer embedding in \tf{ET}. The history answer embeddings are learned.
\end{enumerate}

The second method is \tf{History Attention Mechanism (HAM)}. After extracting the token-level BERT representation from the first step, they run the these representations through a fine-grained history attention net, which computes the attention weights to each previous turn in history for each token in the sequence. The same token might be embedded with different history information, thus having different token representations. These attention weights are on a token level and thus are more fine-grained than those from the sequence-level representations.

The history attention network is a single-layer feed-forward network. It learns an attention vector $\mathbf{D} \in \mathbb{R}^{h}$ to map a token representation $\mathbf{t}_k^i$ to a logit and use the softmax function to compute probabilities across all sequences generated by the same instance. The token-level attention input for the $m$-th token in the sequence is denoted as $\mathbf{t}_k(m) = \{\mathbf{t}_k^i(m)\}_{i=1}^I$, where $\mathbf{t}_k(m) \in \mathbb{R}^{I \times h}$. Then these attention weights are applied to $\mathbf{t}_k(m)$ itself:
\begin{equation}\label{eqn:fine-grained-attention-weights}
\begin{aligned}
& w_i = \frac{e^{\mathbf{D} \cdot \mathbf{t}_k^i(m)}}{\sum_{i'=1}^I e^{\mathbf{D} \cdot \mathbf{t}_k^{i'}(m)}} \\
& \hat{\mathbf{t}}_k(m) = \sum_{i=1}^I \mathbf{t}_k^i(m) \cdot w_i
\end{aligned}
\end{equation}
where $\hat{\mathbf{t}}_k(m) \in \mathbb{R}^{h}$ is the aggregated token representation for the $m$-th token in this sequence. Therefore, the aggregated token-level representation $\hat{\mathbf{T}}_k$ for this sequence is $\{\hat{\mathbf{t}}_k(m)\}_{m=1}^M$.

\paragraph{ExCorD.} For each turn, they augment the question by prepending one previous question-answer pairs to the current question. If training, then they construct a self-contained history by concatenating the self-contained questions with gold answers. and employ consistency regularization by encouraging the model to give the same predictions using original questions with using self-contained questions. If evaluating, then they only use the conversation history constructed with original questions.

\paragraph{GraphFlow.} For each turn, they augment the question by prepending two previous question-answer pairs to the current question. In addition, to each word vector in an augmented question, they concatenate a turn marker embedding $f_{\text{turn}}(q_{k}^{(i)})$ indicating which turn the word belongs to. In short, each question word $q_{k}^{(i)}$ is encoded by a vector $\mf{w}_{q_k}^{(i)}$ which is a concatenation of word embeddings (i.e., $\mf{g}_{k}^{Q^{(i)}}$ and $\text{BERT}_{k}^{Q^{(i)}}$) and turn marker vector $f_{\text{turn}}(q_{k}^{(i)})$.

They also create a feature vector $f_{\text{ans}}(c^{(i)}_{j})$ encoding previous $N$ answer locations to be concatenated to context word embeddings. At the $i$-th turn in a conversation, each context word $c_j$ is encoded by a vector $\mf{w}^{(i)}_{c_j}$ which is a concatenation of linguistic vector $f_{\text{ling}}(c^{(i)}_{j})$ (i.e. POS and NER tagging information), word embeddings (i.e., $\mf{g}_j^C$ and $\text{BERT}_j^C$), aligned vector $f_{\text{align}}(c^{(i)}_{j})$ and previous answer vector $f_{\text{ans}}(c^{(i)}_{j})$.

\subsection{Determining Unanswerable Questions} \label{subsec:unans}

The QuAC dataset concatenates a \unans token to each passage. \bert, \ham and \excord utilize this property by calculating the probability of the \unans token together with other tokens in the passage. \graphflow, however, uses a separate linear layer to calculate the probability of outputting \unans~.

==> tables/BT_result.tex <==
%!TEX root = ../main.tex

\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c|c|c|c}
    \toprule
         & \tf{\bert} & \tf{GF} & \tf{\ham} & \tf{\excord} \\
    \midrule
    Human & 0.144 & 0.145 & 0.350 & 0.361 \\
    \Gold & 0.162 & 0.223 & 0.239 & 0.376  \\
    \Pred & 0.165 & 0.140 & 0.231 & 0.464 \\
    \Replace & 0.162 & 0.157 & 0.231 & 0.451 \\
    \Rewrite &  0.165 & 0.136 & 0.219 & 0.480 \\
    \bottomrule
    \end{tabular}
    }
    \caption{$\lambda_{\model}$ of each model under each metric.}
    \label{tab:bt_result}
\end{table}

==> tables/answerable.tex <==
%!TEX root = ../main.tex

\begin{table*}[t]
\begin{center}
\begin{tabular}{l|c|c|c|c}
\toprule
Evaluation Mode & \textbf{BERT} & \textbf{HAM} & \textbf{ExCorD} & \textbf{GraphFlow} \\
\midrule
Auto-Gold (F1) & 61.8 & 64.5 & 66.4 & 66.6 \\
Auto-Pred (F1) & 52.7 & 54.6 & 59.2 & 54.5 \\
Auto-Filter (F1) & 51.8 & 55.8 & 60.3 & 53.4 \\
\midrule
Human (Accuracy) & 75.9 & 84.8 & 85.3 & 83.2 \\
\bottomrule
\end{tabular}
\end{center}
\caption{F1 score/Accuracy of \textit{answerable questions} of each model under different evaluation mode. For automatic evaluations, we report F1 score of the questions that are answerable according to the original QuAC dataset annotation. For human evaluations, we report accuracy of the questions that are annotated as answerable by crowd workers.}
\label{tab:performance-text_acc_f1}
\end{table*}

==> tables/auto_replace.tex <==
%!TEX root = ../main.tex

\begin{table*}[ht]
\begin{center}
    \resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|cccc|cccc}
\toprule
 & \multicolumn{4}{c|}{\tf{Overall}} &  \multicolumn{4}{c}{\tf{Answerable questions}} \\
 & \textbf{\bert} &\textbf{GF} & \textbf{\ham} & \textbf{\excord} &  \textbf{\bert}& \textbf{GF}  & \textbf{\ham} & \textbf{\excord} \\
\midrule
Auto-Gold (F1) & 63.2 & 64.9 & 65.4 & 67.7 & 61.8 & 66.6  & 64.5 & 66.4 \\
Auto-Pred (F1) & 54.6 & 49.6 & 57.2 & 61.2 &  52.7 & 54.5 & 54.6 & 59.2 \\
Auto-Rewrite (F1) & 54.5 & 48.2 & 57.3 & 61.9 & 51.2 & 51.9 & 55.1 & 59.7  \\
Auto-Replace (F1) & 54.2 & 47.8 & 57.1 & 61.7 & 50.7 & 51.7 & 54.8 & 59.7 \\
\midrule
Human (Accuracy) & 82.6 &81.0 &  87.8 & 87.9 & 75.9 & 83.2 &  84.8 & 85.3 \\
\bottomrule
\end{tabular}}
\end{center}
\caption{F1 score of each model under the each metric.}
\label{tab:replace-acc_f1}
\end{table*}

\begin{table*}[ht]
\begin{center}
\begin{tabular}{l|lcccc}
\toprule
 & \multicolumn{4}{c|}{\textbf{Unanswerable Q}} & \multicolumn{4}{c|}{\textbf{Pred. No Ans.}} & \multicolumn{4}{c|}{\textbf{Precision}} & \multicolumn{4}{c}{\textbf{Recall}} \\
& B & G & H & E & B & G & H & E &  B & G & H & E &  B & G & H & E \\
\midrule
\gold{} & 20.2 & 20.2  & 20.2 & 20.2 & 27.1 & 21.5 & 27.1 & 28.3  & 56.8 & 62.3 & 57.1 & 57.9 & 68.1 & 59.3 & 68.4 & 72.5  \\
\pred{} &  20.2 & 20.2 & 20.2 & 20.2  & 27.8 & 13.8 & 28.6 & 28.9 &  50.0 & 53.9 & 52.3 & 53.3 & 61.4 & 33.0 & 66.1 & 68.2 \\
\rewrite{} &  20.2 & 20.2 & 20.2 & 20.2 & 27.3 & 13.1 & 25.1 & 26.0  & 48.6 & 55.0 & 52.4 & 53.9 &  65.7 & 35.7 & 65.1 & 69.4\\
\replace{} &   20.2 & 20.2 & 20.2 & 20.2  & 27.5 & 12.9 & 25.2 & 25.7  & 48.6 & 54.2 & 52.1 & 53.8 & 66.1 & 34.7 & 64.9 & 68.4 \\
\midrule
Human & 34.6 & 20.6 & 34.1 & 33.2 & 42.3 & 14.7 & 37.2 & 36.0 & 75.0 & 93.0 & 86.8 & 87.4  & 95.2 & 72.5 & 93.7 & 93.3 \\
% & Metrics & \textbf{\bert} & \textbf{GF} & \textbf{\ham} & \textbf{\excord} \\
% \midrule
% \multirow{ 4}{*}{Auto-Gold} & Unanswerable Q (\%) & 20.2 & 20.2  & 20.2 & 20.2 \\
% & Pred. No Ans. (\%) & 27.1 & 21.5 & 27.1 & 28.3 \\
% & Precision (\%) & 56.8 & 62.3 & 57.1 & 57.9 \\
% & Recall (\%) & 68.1 & 59.3 & 68.4 & 72.5  \\
% \midrule
% \multirow{ 4}{*}{Auto-Pred} & Unanswerable Q (\%) & 20.2 & 20.2 & 20.2 & 20.2  \\
% & Pred. No Ans. (\%) & 27.8 & 13.8 & 28.6 & 28.9 \\
% & Precision (\%) & 50.0 & 53.9 & 52.3 & 53.3 \\
% & Recall (\%) & 61.4 & 33.0 & 66.1 & 68.2  \\
% \midrule
% \multirow{ 4}{*}{Auto-Rewrite} & Unanswerable Q (\%) &  20.2 & 20.2 & 20.2 & 20.2  \\
% & Pred. No Ans. (\%) & 27.3 & 13.1 & 25.1 & 26.0 \\
% & Precision (\%) & 48.6 & 55.0 & 52.4 & 53.9 \\
% & Recall (\%) & 65.7 & 35.7 & 65.1 & 69.4 \\
% \midrule
\multirow{ 4}{*}{Auto-Replace} & Unanswerable Q (\%) &  20.2 & 20.2 & 20.2 & 20.2  \\
& Pred. No Ans. (\%) & 27.5 & 12.9 & 25.2 & 25.7 \\
& Precision (\%) & 48.6 & 54.2 & 52.1 & 53.8 \\
& Recall (\%) & 66.1 & 34.7 & 64.9 & 68.4 \\
\midrule
% \multirow{ 4}{*}{Human} & Unanswerable Q (\%) & 34.6 & 20.6 & 34.1 & 33.2 \\
% & Pred. No Ans. (\%) & 42.3 & 14.7 & 37.2 & 36.0 \\
% & Precision (\%) & 75.0 & 93.0 & 86.8 & 87.4 \\
% & Recall (\%) & 95.2 & 72.5 & 93.7 & 93.3 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Statistics of unanswerable questions of each model under each metric.}
\label{tab:replace-unans}
\end{table*}

\begin{table*}[ht]
    \centering
    \begin{tabular}{l|c|c|c|c}
    \toprule
    Pair & \Gold & \Pred & \Rewrite & \Replace\\
    \midrule
    B/E & 52.0 & 58.0 & 62.0 & 65.0 \\
    H/B & 52.0 & 53.0 & 57.0 & 51.0 \\
    H/E & 45.0 & 48.0 & 52.0 & 49.0 \\
    G/B & 43.4 & 50.5 & 50.5 & 50.5 \\
    G/E & 52.5 & 67.7 & 57.8 & 56.6 \\
    G/H & 44.4 & 62.6 & 58.6 & 57.6 \\
    \bottomrule
    \end{tabular}
    \caption{Agreement (\%) of each automatic evaluation metric in pairwise ranking of different models.}
    \label{tab:replace-align}
\end{table*}


==> tables/errors.tex <==
\begin{table*}[ht]
\begin{center}
\begin{tabular}{c|c|c}  
\toprule
Error Category & Error Reason & \% \\
\midrule
\multirow{4}{*}{Wrong coreference} & Wrong prediction & 18.4 \\
 & No prediction & 4.4 \\
 & Extra gold Information & 6.3 \\
 & Open question & 17.1 \\
\midrule
\multirow{4}{*}{Incoherence} & Wrong prediction & 10.8 \\
 & No prediction & 9.5 \\
 & Extra gold Information & 7.0 \\
 & Open question & 10.1\\
\midrule
Gold answer changed & n/a & 17.7 \\
Missing context & n/a & 3.8 \\
\midrule
\multicolumn{2}{c|}{Total problematic questions} & 158\\
\multicolumn{2}{c|}{Total turns} & 718\\
\multicolumn{2}{c|}{Error Rate} & 22\\
\bottomrule
\end{tabular}
\end{center}
\caption{Error categories and reasons for 100 passages sampled from QuAC dataset. 
\tianyu{This table seems too large. Do you think we can have a pie chart for this and take only one column?} \huihan{See Figure \ref{fig:error_categories}}
\tianyu{Another problem: I think this should be a 4x4 table to be honest. Or we can just disentangle this table.}
}
\label{tab:error_categories}
\end{table*}

==> tables/eval_statistics.tex <==
%!TEX root = ../main.tex

\begin{table*}[t]
\begin{center}
\begin{tabular}{l|c c c c}
\toprule
Evaluation Mode & \textbf{BERT} & \textbf{HAM} & \textbf{ExCorD} & \textbf{GraphFlow} \\
\midrule
\#Passage & \multicolumn{4}{c}{1,000} \\
Auto-Gold \#Q &  \multicolumn{4}{c}{7,354}\\
Auto-Pred \#Q &  \multicolumn{4}{c}{7,354}\\
Auto-Filter \#Q & 6,309 & 6,296 & 6,339 & 6,308 \\
\midrule
Human \#Passage & 100 & 100 & 100 & 100 \\
Human \#Q  & 3,767 & 3,978 & 3,683 & 3,670\\
\bottomrule
\end{tabular}
\end{center}
\caption{Number of questions and passages used for each automatic evaluation mode and human evaluation mode. For human evaluation, we collect three conversations for each passage in the QuAC dataset. }
\label{tab:overall-statistics}
\end{table*}

==> tables/filter_stat.tex <==
%!TEX root = ../main.tex

\begin{table}[t]

\begin{center}
\resizebox{0.98\columnwidth}{!}{
\begin{tabular}{l|c c c c}
\toprule
 & \tf{\bert} &\tf{GF} & \tf{\ham} & \tf{\excord} \\
\midrule
Rewritten \#Q & 12.2\% &  13.3\%  & 12.4\% & 11.9\% \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Percentage of questions detected as invalid and rewritten by our \rewrite{} protocol.
}
\label{tab:filter_stats}

\end{table}

==> tables/gold_answer_changed.tex <==
%!TEX root = ../main.tex

\begin{figure}[ht]
    \centering
    \resizebox{0.95\columnwidth}{!}
    {\begin{tabular}{cl}
    \toprule
        Q5: & Were they successful in their attempts to \\
        & circumnavigate the globe?\\
        G5: & they made a record-breaking flight from \\
        & Morocco to Hawaii but were unable to complete \\
        & a global flight\\
        P5: & while successfully crossing the channel, \\
        & did not break Branson's record. \\\\
        Q6: & What were some problems they encountered?\\
    \bottomrule
    \end{tabular}
    }
    \caption{Correct answer changed: The correct answers to Q6 based on G5 or P5 are expected to be different.}
    \label{tab:gold_answer_changed}
\end{figure}


==> tables/intro_drop.tex <==
%!TEX root = ../main.tex

\begin{table}[ht]
    \begin{center}
    \centering
    \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \tf{Type of Answer} & \tf{BERT} & \tf{HAM} & \tf{ExCorD} & \tf{GraphFlow}\\
    \midrule
        Gold & 63.2 & 65.4 & 67.7 & 64.9\\
        Predicted & 54.6 & 57.2 & 61.2 & 49.6\\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{
        Significant drop in F1 score of using the QuAC development set. Different models are affected by the cascaded error differently. The relative ranking of models also change when switched to predicted answers. \danqi{This table is too small and is not super informative. Can we add human evaluations here too? Can we visualize them, instead of presenting them in a table?}}
    \label{tab:cascaded}
\end{table}


==> tables/missing_context.tex <==
%!TEX root = ../main.tex

\begin{table}[ht]
    \centering
    \resizebox{0.95\columnwidth}{!}
    {
    \begin{tabular}{cl}
    \toprule
        Q7: &  Can you tell me any other information? \\
        G7: & Vachel Lindsay’s “singing poem” “Bryan, \\
        & Bryan, Bryan, Bryan” is a lengthy tribute to \\
        & the idol of the poet’s youth. \\
        P7: & L. Frank Baum satirized Bryan as the \\
        & Cowardly Lion in The Wonderful Wizard of Oz, \\
        & published in 1900. \\\\
        Q8: & What did Bryan mean to Vachel? \\
    \bottomrule
    \end{tabular}
    }
    \caption{Q8 is unanswerable without knowing the relationship between "Bryan" and "Vachel", which can only be inferred from G7. This contextual information is not provided from P7.}
    \label{tab:missing_context}
\end{table}


==> tables/not_coherent.tex <==
%!TEX root = ../main.tex

\begin{figure}[ht]
    \centering
    \resizebox{0.95\columnwidth}{!}
    {\begin{tabular}{cl}
    \toprule
        Q3: & Did he succeed in becoming a chaplain? \\
        G3: & he contracted mumps shortly after applying \\
        & for a commission. \\
        P3: & After a period of recuperation in Florida, \\
        & he was hired as the first full-time evangelist \\
        & of the new Youth for Christ \\\\
        Q4: & Did he retire after his mumps diagnosis? \\
    \bottomrule
    \end{tabular}
    }
    \caption{Incoherence: Q4 asks about "mumps diagnosis", which is a follow up on G3. While Q4 can be answered solely based on the passage, this question should not be asked based on P3.}
    \label{tab:not_coherent}
\end{figure}


==> tables/pairwise_pred.tex <==
%!TEX root = ../main.tex

\begin{table*}[ht]
\begin{center}
\begin{tabular}{c|c|c|c|c}
\toprule
Models & BERT & HAM & ExCorD & Graphflow \\
\midrule
BERT & - & 58\% & 59\% & 47\% \\
\midrule
HAM & 58\% & - & 47\% & 60\% \\
\midrule
ExCorD  & 59\% & 47\% & - & 65\% \\
\midrule
Graphflow  & 47\% & 60\% & 65\% & - \\
\bottomrule
\end{tabular}
\end{center}
\caption{Pairwise agreement between human evaluation and automatic evaluation using predicted history}
\label{tab:pairwise_pred}
\end{table*}


==> tables/rewrite_example.tex <==
%!TEX root = ../main.tex

\begin{figure}[t]
    \centering
    \resizebox{0.98\columnwidth}{!}
    {\begin{tabular}{ll}
    \toprule

    % \midrule
        $Q^*_1$: & What does the article say about RoadMaster? \\
        $A^*_1$: & In 1972, Clark attempted to record \\
        &  {\color{orange}a follow-up album}. Progress was slow and \\
        &  expensive, and {\color{purple}A\&M} terminated the project  \\
        &  before completion. \\
        $A_1$: & CANNOTANSWER \\

        ~\vspace{-8pt}\\
        $Q^*_2$: & Why did they terminate the project? \\
        $\hat{Q}_2$: & Why did {\color{purple}A\&M} terminate {\color{orange}a follow-up album}? \\
    \bottomrule
    \end{tabular}
    }
    \caption{
    An example of correctly captured and rewritten invalid question by Auto-Rewrite.
    }
    \label{tab:exp_of_rewrite}
\end{figure}


==> tables/wrong_coref.tex <==
%!TEX root = ../main.tex

\begin{figure}[ht]
    \centering
    \resizebox{0.62\columnwidth}{!}
    {\begin{tabular}{cl}
    \toprule
        Q1: & What was their first song?\\
        G1: & Punch in the Face\\
        P1: & \unans \\\\
        Q2: & How did \textbf{it} fair?\\
    \bottomrule
    \end{tabular}
    }
    \caption{Unresolved coreference: "It" in Q2 cannot be resolved from predicted history (Q1, P1) because the pronoun refers to the entity in G1.}
    \label{tab:wrong_coref}
\end{figure}
